On the Optimal Weighted $\ell_2$ Regularization in Overparameterized Linear Regression

We consider the linear model $\mathbf{y} = \mathbf{X} \mathbf{\beta}_\star + \mathbf{\epsilon}$ with $\mathbf{X}\in \mathbb{R}^{n\times p}$ in the overparameterized regime $p>n$. We estimate $\mathbf{\beta}_\star$ via generalized (weighted) ridge regression: $\hat{\mathbf{\beta}}_\lambda = \left(\mathbf{X}^T\mathbf{X} + \lambda \mathbf{\Sigma}_w\right)^\dagger \mathbf{X}^T\mathbf{y}$, where $\mathbf{\Sigma}_w$ is the weighting matrix. Under a random design setting with general data covariance $\mathbf{\Sigma}_x$ and anisotropic prior on the true coefficients $\mathbb{E}\mathbf{\beta}_\star\mathbf{\beta}_\star^T = \mathbf{\Sigma}_\beta$, we provide an exact characterization of the prediction risk $\mathbb{E}(y-\mathbf{x}^T\hat{\mathbf{\beta}}_\lambda)^2$ in the proportional asymptotic limit $p/n\rightarrow \gamma \in (1,\infty)$. Our general setup leads to a number of interesting findings. We outline precise conditions that decide the sign of the optimal setting $\lambda_{\rm opt}$ for the ridge parameter $\lambda$ and confirm the implicit $\ell_2$ regularization effect of overparameterization, which theoretically justifies the surprising empirical observation that $\lambda_{\rm opt}$ can be negative in the overparameterized regime. We also characterize the double descent phenomenon for principal component regression (PCR) when both $\mathbf{X}$ and $\mathbf{\beta}_\star$ are anisotropic. Finally, we determine the optimal weighting matrix $\mathbf{\Sigma}_w$ for both the ridgeless ($\lambda\to 0$) and optimally regularized ($\lambda = \lambda_{\rm opt}$) case, and demonstrate the advantage of the weighted objective over standard ridge regression and PCR.

==> proof.tex <==
\section{Proofs}
Note that from \eqref{eq:derivative} (with $\zeta$ replaced by $\zeta_r$), we know the optimal $\lambda_{\opt}$ should satisfies that
\begin{eqnarray}
    \frac{\tilde{\sigma}^2+\gamma \bbE\frac{g(V)h(V)}{(\zeta_r+1)^2}}{1-\gamma \bbE\frac{\zeta_r^2}{(1+\zeta_r)^2}} \ = \ \frac{\bbE \frac{g(V)h(V)\zeta_r}{(1+\zeta_r)^3}}{\bbE \frac{\zeta_r^2}{(1+\zeta_r)^3}}.
\end{eqnarray}








Hence, we have
\[
R(r,\lambda_{\opt})\ = \ \frac{\bbE \frac{g(V)h(V)\zeta_r}{(1+\zeta_r)^3}}{\bbE \frac{\zeta_r^2}{(1+\zeta_r)^3}}.
\]


Hence, with Jensen's inequality, we can upper bound the denominator of the risk function
\[
1-\gamma\bbE\frac{\zeta^2}{(1+\zeta)^2} \leq 1- \gamma \left(\bbE\frac{\zeta}{1+\zeta}\right)^2 = 1-\frac{1}{\gamma}\left(1-\lambda m_r(-\lambda)\right)^2
\]
On the other hand, when $g(V)h(V)$ and $r(V)$ have different monotonicity of $V$, we can lower bound the numerator of the risk function:
\[
\tilde{\sigma}^2+\gamma \bbE\frac{g(V)h(V)}{(1+\zeta)^2} \geq \tilde{\sigma}^2 +\gamma \bbE g(v)h(V) \bbE\frac{1}{(1+\zeta)^2}\geq
\tilde{\sigma}^2 +\frac{1}{\gamma} \bbE g(v)h(V)\left(\gamma-1+\lambda m(-\lambda)\right)^2
\]



WLOG, we assume that $h\in\cH_I^{+}$ and $g\in\cH_I$. Then our first step is to show that the optimal $r\in \cH_I^{+}\bigcup\cH_D^{+}$ should belong to $\cH_I^{+}$.
........


Hence, we just need to focus on all possible $r\in\cH_{I}^{+}$.  

\begin{eqnarray}
R_{\alpha}(\lambda)\ \triangleq \ \frac{m'_{\alpha}(-\lambda)}{m^2_{\alpha}(-\lambda)}\left(\tilde{\sigma}^2+\gamma \bbE\frac{g(V)h(V)}{(r_{\alpha}(V)m_{\alpha}(-\lambda)+1)^2}\right),\n
\end{eqnarray}



Note that when $\alpha=0$, we have $R_0(\lambda)$ being the risk function for $\vSigma_w=\tilde{\vSigma}_w$ and when $\alpha=1$, we have $R_1(\lambda)$ being the risk function for $\vSigma_w=\vSigma_{\beta}^{-1}$\footnote{For any $\alpha\in(0,1)$, the risk function $R(\alpha)$ is well defined but it may not be the limit of the expected risk for any choice of $\vSigma_w$ unless $r\in\cH_{I}^{+}$}.
Our goal is to show that $\alpha=1$ is a first order stationary point for optimizing the optimal weighted ridge regression i.e., $\min_{\alpha}\min_{\lambda}R_{\alpha}(\lambda)$. Simiarly as 

Then, the risk function can be equivalently expressed by the following formula:
\begin{eqnarray}
R_{\alpha}(\lambda_{\opt}) &=& \frac{\tilde{\sigma}^2+\gamma \bbE\frac{g(V)h(V)}{(\zeta_{\alpha}+1)^2}}{1-\gamma \bbE\frac{\zeta_{\alpha}^2}{(1+\zeta_{\alpha})^2}}\label{eq:R_alpha}
\end{eqnarray}

Hence, we have
\[
R_{\alpha}(\lambda_{\opt})\ = \ \frac{\bbE \frac{g(V)h(V)\zeta_{\alpha}}{(1+\zeta_{\alpha})^3}}{\bbE \frac{\zeta_{\alpha}^2}{(1+\zeta_{\alpha})^3}}.
\]
With \eqref{eq:m'alpha}, we have
\begin{eqnarray}
\frac{\dif R_{\alpha}(\lambda_{\opt})}{\dif \alpha}&\stackrel{(i)}{\propto_+}&\left(\bbE\frac{\zeta_{\alpha}}{(1+\zeta_{\alpha})^2}\bbE\frac{\psi_{\alpha}(1-2\zeta_{\alpha})(\psi_{\alpha}-\zeta_{\alpha})}{(1+\zeta_{\alpha})^4}-\bbE\frac{\psi_{\alpha}\zeta_{\alpha}(1-2\zeta_{\alpha})}{(1+\zeta_{\alpha})^4}\bbE\frac{\psi_{\alpha}-\zeta_{\alpha}}{(1+\zeta_{\alpha})^2}\right)\bbE\frac{\zeta_{\alpha}^2}{(1+\zeta_{\alpha})^3}\n\\
&&-\left(\bbE\frac{\zeta_{\alpha}}{(1+\zeta_{\alpha})^2}\bbE\frac{\zeta_{\alpha}(2-\zeta_{\alpha})(\psi_{\alpha}-\zeta_{\alpha})}{(1+\zeta_{\alpha})^4}-\bbE\frac{\zeta_{\alpha}^2(2-\zeta_{\alpha})}{(1+\zeta_{\alpha})^4}\bbE\frac{\psi_{\alpha}-\zeta_{\alpha}}{(1+\zeta_{\alpha})^2}\right)\bbE\frac{\psi_{\alpha}\zeta_{\alpha}}{(1+\zeta_{\alpha})^3}.\n\\
\end{eqnarray}
where in equation (i) we have omitted the following positive quantity
\[
\left((1-\alpha)m_{\alpha}(-\lambda)\left(\bbE \frac{\zeta_{\alpha}^2}{(1+\zeta_{\alpha})^3}\right)^2\bbE\frac{\zeta_{\alpha}}{(1+\zeta_{\alpha})^2}\right)^{-1}
\]



\begin{itemize}
    \item When $h(v)g(v)\in \cH_I$, then the optimal choice of $r\in \cH_{I}\bigcup\cH_D$ belongs to $\cH_I$.
    \item When $h(v)g(v)\in \cH_D$, then the optimal choice of $r\in \cH_{I}\bigcup\cH_D$ belongs to $\cH_D$.
\end{itemize}
Further, $r(v)\stackrel{\text{a.s.}}{=} h(v)g(v)$ with respect to $V$ is a first order stationary point


In general, the sufficient condition to have negative optimal regularization is the following:
\[
\bbE \frac{g(V)\zeta^2}{(1+\zeta)^3}\bbE\frac{\zeta}{(1+\zeta)^2}>\bbE g(V)\left(\frac{\zeta}{(1+\zeta)^2}+\frac{\zeta}{\gamma\xi}\right)\bbE\frac{\zeta^2}{(1+\zeta)^3}.
\]


Further, for special case when $\tilde{\sigma}^2=0$ and $\vSigma_x=\vSigma_{\beta}^{-1}$(i.e., $h(v)g(v)\equiv 1$), we can confirm that the minimal risk is $\gamma$ for the regime $\theta\gamma<1$ while the risk achieved at $\theta=1$ 
at full model is $\gamma-1$ while the optimal under-parameterized regime is $\gamma$.


Note that from \eqref{eq:smrelation}, we have
\[
    0<\gamma s(-\lambda) = m(-\lambda)-\frac{1-\gamma}{\lambda} = \frac{\gamma \bbE\frac{1}{1+\zeta}}{\lambda},
\]
where the last equality holds due to \eqref{eq:relation_m}. Hence, we have
\begin{eqnarray}
\bbE \frac{1}{1+h(V)m(-\lambda)} < 0, \quad \forall \lambda<0.
\label{eq:under_eq_1}
\end{eqnarray}
Note that the support of $V$ is a single point or interval and $h$ is a continuous function, which means $\bbE \frac{1}{1+h(V)m(-\lambda)}$ is only valid when either $1+h(V)m(-\lambda)<0$ or $1+h(V)m(-\lambda)>0$ holds almost surely with respect to $V$. Hence, due to \eqref{eq:under_eq_1}, we have $1+h(V)m(-\lambda)<0$ holds almost surely if $\lambda<0$ and $m(-\lambda)<0$. Therefore, for the case when $\lambda<0$ and $m(-\lambda)<0$, we have
\[
\bbE\frac{h^2(V)}{(1+h(V)m(-\lambda))^3} < 0,
\]
and \eqref{eq:under_goal_1} holds. 
